How to Perform Distributed Precoding to Wirelessly Power Shelf Labels: Signal Processing and Measurements

Wireless power transfer (WPT) has garnered increasing attention due to its potential to eliminate device-side batteries. With the advent of (distributed) multiple-input multiple-output (MIMO), radio frequency (RF) WPT has become feasible over extended distances. This study focuses on optimizing the energy delivery to Energy Receivers (ERs) while minimizing system total transmit power. Rather than continuous power delivery, we optimize the precoding weights within specified time slots to meet the energy requirements of the ERs. Both unsynchronized (non-coherent) and synchronized (coherent) systems are evaluated. Our analysis indicates that augmenting the number of antennas and transitioning from an unsynchronized to asynchronized full phase-coherent system substantially enhances system performance. This optimization ensures precise energy delivery, reducing overshoots and overall energy consumption. Experimental validation was conducted using a testbed with84 antennas, validating the trends observed in our numerical simulations.

==> figures/techtile/non-coherent/partial-power-tx.tex <==
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={M},
xmajorgrids,
xmin=-3.1, xmax=87.1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Power [W]},
ymajorgrids,
ymin=3.95, ymax=5.4,
ytick style={color=black}
]


\draw[black, semithick,fill=black!5, fill opacity=0.8] (2,4.06) rectangle (84,4.24); %



\addplot [semithick, steelblue31119180] table [col sep=space, x=x, y=y] {figures/techtile/non-coherent/partial-power-tx.dat};


\draw[black, semithick] (2,0.92) -- (21,1.132); %

\draw[black, semithick] (84,0.92) -- (78.8,1.132); %


\end{axis}

 \begin{axis}[xmin=2,xmax=84,ymin=4.06,ymax=4.24,grid,height=4cm,width=6cm,
            shift={(1.8cm,2.5cm)},axis background/.style={fill=black!3}]
            \addplot[semithick, steelblue31119180] table [col sep=space, x=x, y=y] {figures/techtile/non-coherent/partial-power-tx.dat};
\end{axis}            

\end{tikzpicture}


==> figures/techtile/rx-cdf-coherent.tex <==
\addplot [thick, dashed, steelblue31119180]
table {%
1.18256000000001 0
1.18256000000003 0.00416666666666667
1.18256000000061 0.00833333333333333
1.1825600000014 0.0125
1.25616903023497 0.0166666666666667
1.35425343521356 0.0208333333333333
1.38952471039399 0.025
1.38985325330699 0.0291666666666667
1.42042782424437 0.0333333333333333
1.44619935755021 0.0375
1.46705316640915 0.0416666666666667
1.47634347907456 0.0458333333333333
1.48496330996389 0.05
1.48527248458482 0.0541666666666667
1.49348005475034 0.0583333333333333
1.49430700729151 0.0625
1.51153346669793 0.0666666666666667
1.53367142398698 0.0708333333333333
1.61105692420692 0.0791666666666667
1.62416743331447 0.0833333333333333
1.62537891208648 0.0875
1.64585978803752 0.0916666666666667
1.70030639398151 0.0958333333333333
1.7039539074131 0.1
1.73947983147462 0.104166666666667
1.74991982469206 0.108333333333333
1.7610685224023 0.1125
1.80633431699185 0.116666666666667
1.8159633502082 0.120833333333333
1.83088858327781 0.125
1.83636576258377 0.129166666666667
1.84296812251201 0.133333333333333
1.85025794596512 0.1375
1.87347676577644 0.141666666666667
1.90074695573322 0.145833333333333
1.9030757600431 0.15
1.90917200815376 0.154166666666667
1.91502645224127 0.158333333333333
1.92346830290612 0.1625
1.94696326693757 0.166666666666667
1.95984242317373 0.170833333333333
1.98900145303223 0.175
1.99561741980217 0.179166666666667
2.02394637288083 0.183333333333333
2.03562041520639 0.1875
2.03784896312728 0.191666666666667
2.06473516190949 0.195833333333333
2.10582976537159 0.2
2.14095335950981 0.204166666666667
2.14936984606943 0.208333333333333
2.16548170102338 0.2125
2.17456186335315 0.216666666666667
2.20548891764624 0.220833333333333
2.21940289745384 0.225
2.2218960403879 0.229166666666667
2.24106112043168 0.233333333333333
2.2462658557648 0.2375
2.24730137693976 0.241666666666667
2.26382515421789 0.245833333333333
2.28108079964205 0.25
2.28746452072334 0.254166666666667
2.34771595413816 0.258333333333333
2.37289943855332 0.2625
2.38071561469779 0.266666666666667
2.40198063600584 0.270833333333333
2.40757942894574 0.275
2.42660037754035 0.279166666666667
2.44477663428119 0.283333333333333
2.48563762857192 0.2875
2.50432910053413 0.291666666666667
2.51072073774494 0.295833333333333
2.52347146291416 0.3
2.53751080463994 0.304166666666667
2.54286298805081 0.308333333333333
2.55425038652164 0.3125
2.55905520513041 0.316666666666667
2.56509743848128 0.320833333333333
2.56713810376966 0.325
2.57886211688788 0.329166666666667
2.57983667846112 0.333333333333333
2.58915243677602 0.3375
2.59612395188956 0.341666666666667
2.59764140617961 0.345833333333333
2.60961792346017 0.35
2.62645016918232 0.354166666666667
2.62765136788236 0.358333333333333
2.66634516120459 0.3625
2.67595643529722 0.366666666666667
2.68217409122217 0.370833333333333
2.71688567247071 0.375
2.7682066132475 0.379166666666667
2.77090170194621 0.383333333333333
2.78593204514651 0.3875
2.78956261836994 0.391666666666667
2.79135182900912 0.395833333333333
2.80090041911707 0.4
2.80140306431245 0.404166666666667
2.80889738472277 0.408333333333333
2.81256544513593 0.4125
2.81609249234033 0.416666666666667
2.81676218418394 0.420833333333333
2.85524543882432 0.425
2.85777562597856 0.429166666666667
2.85805847973851 0.433333333333333
2.85833942395626 0.4375
2.86418507852148 0.441666666666667
2.86511745720233 0.445833333333333
2.87283074675978 0.45
2.87432836400899 0.454166666666667
2.89796158187357 0.458333333333333
2.90943074098753 0.4625
2.92153782951485 0.466666666666667
2.95047488316461 0.470833333333333
2.98049240101154 0.475
2.99001511998468 0.479166666666667
3.00736334036519 0.483333333333333
3.01441733867754 0.4875
3.02873361727978 0.491666666666667
3.02892963483429 0.495833333333333
3.06519249333107 0.5
3.08816280293114 0.504166666666667
3.09118273547047 0.508333333333333
3.13505603010479 0.5125
3.1378397131295 0.516666666666667
3.13874674733942 0.520833333333333
3.14032318504166 0.525
3.15573404903425 0.529166666666667
3.16235525089165 0.533333333333333
3.17563442484178 0.5375
3.19321499498363 0.541666666666667
3.20131097480711 0.545833333333333
3.24413343684952 0.55
3.3140384256653 0.554166666666667
3.33376572681996 0.558333333333333
3.3352661103446 0.5625
3.3401358459579 0.566666666666667
3.35676520533573 0.570833333333333
3.36804426224671 0.575
3.45209901870256 0.579166666666667
3.46842380821081 0.583333333333333
3.53704109494583 0.5875
3.57574584190966 0.591666666666667
3.57945747165733 0.595833333333333
3.60411344894145 0.6
3.60621720141908 0.604166666666667
3.63304401571362 0.608333333333333
3.6335371823615 0.6125
3.64416381712714 0.616666666666667
3.66945354527607 0.620833333333333
3.69622835931834 0.625
3.70413061979215 0.629166666666667
3.74205640438335 0.633333333333333
3.75973111555416 0.6375
3.77976956948551 0.641666666666667
3.80332984318641 0.645833333333333
3.8251336904562 0.65
3.85612137048329 0.654166666666667
3.86817331768521 0.658333333333333
3.92046606046409 0.6625
3.92375324251142 0.666666666666667
3.93039338742022 0.670833333333333
3.96857352928466 0.675
3.99527112325858 0.679166666666667
4.0375270592951 0.683333333333333
4.0512073837521 0.6875
4.05865513713555 0.691666666666667
4.07308782485684 0.695833333333333
4.09250324055067 0.7
4.10826360606028 0.704166666666667
4.16340480607955 0.708333333333333
4.17175402906468 0.7125
4.19724451888759 0.716666666666667
4.22111652160624 0.720833333333333
4.24359443504939 0.725
4.2804043017074 0.729166666666667
4.30493775890586 0.733333333333333
4.312434635432 0.7375
4.32886486721625 0.741666666666667
4.3441927244918 0.745833333333333
4.41814532579378 0.75
4.50260670786431 0.754166666666667
4.53582387660567 0.758333333333333
4.5908142373748 0.7625
4.61880001595255 0.766666666666667
4.622763833065 0.770833333333333
4.6311638964446 0.775
4.68068934923806 0.779166666666667
4.7803737395864 0.783333333333333
4.79823747454773 0.7875
4.88311159648701 0.791666666666667
4.90388801513144 0.795833333333333
4.94771820359996 0.8
4.94946465758336 0.804166666666667
5.02596410952372 0.808333333333333
5.02914362200811 0.8125
5.03017828015894 0.816666666666667
5.03445803114531 0.820833333333333
5.14891642757539 0.825
5.24637991730488 0.829166666666667
5.36453086206572 0.833333333333333
5.39070766793596 0.8375
5.44969675909075 0.841666666666667
5.69167216940336 0.845833333333333
5.71833344558629 0.85
5.771038559776 0.854166666666667
5.82734496503747 0.858333333333333
5.85414812299668 0.8625
6.14408644349389 0.866666666666667
6.15202192823632 0.870833333333333
6.44385915231978 0.875
6.54885544319702 0.879166666666667
6.71139851348473 0.883333333333333
6.86232356141053 0.8875
7.31804149808427 0.891666666666667
7.43408020260817 0.895833333333333
7.53340960190498 0.9
7.59381137317763 0.904166666666667
7.61063218887171 0.908333333333333
7.85535490246185 0.9125
7.904505281332 0.916666666666667
8.36650659050352 0.920833333333333
8.52543206714089 0.925
8.53622521726956 0.929166666666667
8.77829228116671 0.933333333333333
9.44856192339653 0.9375
9.85201315969803 0.941666666666667
9.89193555612263 0.945833333333333
10.4404174018929 0.95
10.9480590918394 0.954166666666667
11.3907343102333 0.958333333333333
11.4023930808264 0.9625
11.8054744514153 0.966666666666667
12.050916391239 0.970833333333333
12.4486805431111 0.975
13.4335079155703 0.979166666666667
14.0920820177495 0.983333333333333
15.9745516943683 0.9875
17.9748804406861 0.991666666666667
18.8479415631151 0.995833333333333
};
\addplot [thick,  dashed, darkorange25512714]
table {%
1.18256000000409 0
1.18256000004805 0.00416666666666667
1.18256000006778 0.00833333333333333
1.18256000012707 0.0125
1.18256000029822 0.0166666666666667
1.18256000030298 0.0208333333333333
1.18256000035422 0.025
1.1825600003671 0.0291666666666667
1.18256000038254 0.0333333333333333
1.18256000038517 0.0375
1.18256000041393 0.0416666666666667
1.18256000046289 0.0458333333333333
1.1825600004683 0.05
1.18256000049417 0.0541666666666667
1.18256000049774 0.0583333333333333
1.1825600005834 0.0625
1.18256000068682 0.0666666666666667
1.18256000076393 0.0708333333333333
1.18256000086288 0.075
1.1825600009754 0.0791666666666667
1.18256000119002 0.0833333333333333
1.18256000119043 0.0875
1.1825600012158 0.0916666666666667
1.18256000122712 0.0958333333333333
1.18256000136021 0.1
1.18256000142592 0.104166666666667
1.18256000145076 0.108333333333333
1.18256000168841 0.1125
1.18256000188998 0.116666666666667
1.18256000197839 0.120833333333333
1.1825600020146 0.125
1.18256000210737 0.129166666666667
1.18256000232932 0.133333333333333
1.18256000264352 0.1375
1.18256000267119 0.141666666666667
1.18256000283894 0.145833333333333
1.1825600028866 0.15
1.18256000293082 0.154166666666667
1.1825600029971 0.158333333333333
1.18256000321964 0.1625
1.18256000478889 0.166666666666667
1.18256000553539 0.170833333333333
1.18256000564808 0.175
1.1825600079898 0.179166666666667
1.18256000910479 0.183333333333333
1.18256001504572 0.1875
1.1825600167242 0.191666666666667
1.18256003723334 0.195833333333333
1.18256004322258 0.2
1.18256017251629 0.204166666666667
1.18256203645301 0.208333333333333
1.18401225103724 0.2125
1.1890074451667 0.216666666666667
1.1983767057468 0.220833333333333
1.2008999159372 0.225
1.21335893615764 0.229166666666667
1.2483380021538 0.233333333333333
1.24906267025437 0.2375
1.26263808537977 0.241666666666667
1.26828355345789 0.245833333333333
1.27536849895979 0.25
1.28095406566368 0.254166666666667
1.28718559614614 0.258333333333333
1.29479797241338 0.2625
1.30994000445653 0.266666666666667
1.31138313446291 0.270833333333333
1.31262145656626 0.275
1.31436264190455 0.279166666666667
1.31484895301243 0.283333333333333
1.32461562400044 0.2875
1.33318539452773 0.291666666666667
1.33591943586492 0.295833333333333
1.33667896426527 0.3
1.34725293498846 0.304166666666667
1.34878090618359 0.308333333333333
1.37464389566866 0.3125
1.37601269712758 0.316666666666667
1.39078644466285 0.320833333333333
1.39873846700153 0.325
1.4113144555309 0.329166666666667
1.46983549375689 0.333333333333333
1.53099738865454 0.3375
1.54965192653023 0.341666666666667
1.56516415256476 0.345833333333333
1.57990536568766 0.35
1.58204296026749 0.354166666666667
1.58477091690546 0.358333333333333
1.5955460674941 0.3625
1.64196517323244 0.366666666666667
1.64560553939835 0.370833333333333
1.65747179440836 0.375
1.65939445112207 0.379166666666667
1.66902193269672 0.383333333333333
1.68456814715679 0.3875
1.68760479978793 0.391666666666667
1.68950461356119 0.395833333333333
1.70397085523217 0.4
1.71081712093147 0.404166666666667
1.71417811983379 0.408333333333333
1.73257306697502 0.4125
1.7389044362511 0.416666666666667
1.74397385898773 0.420833333333333
1.74650534714417 0.425
1.74836083650624 0.429166666666667
1.76584199450494 0.433333333333333
1.80862688168602 0.4375
1.81167507801011 0.441666666666667
1.81771887460344 0.445833333333333
1.82331442108594 0.45
1.82515036397662 0.454166666666667
1.82873305978872 0.458333333333333
1.83451348678696 0.4625
1.84499156047085 0.466666666666667
1.84660006439311 0.470833333333333
1.85658675390453 0.475
1.86766523513095 0.479166666666667
1.86973910119447 0.483333333333333
1.88085850110034 0.4875
1.88322191703774 0.491666666666667
1.88787600500947 0.495833333333333
1.88970403020814 0.5
1.91121010815789 0.504166666666667
1.92316478151738 0.508333333333333
1.92326801299649 0.5125
1.93584143452128 0.516666666666667
1.93698644975619 0.520833333333333
1.94353584752759 0.525
1.94696400037232 0.529166666666667
1.95123479625611 0.533333333333333
1.95965022832544 0.5375
2.00919412216995 0.541666666666667
2.02578326011137 0.545833333333333
2.0374795025274 0.55
2.03817073602097 0.554166666666667
2.06283741291368 0.558333333333333
2.06814223409151 0.5625
2.06966408116059 0.566666666666667
2.07098252803819 0.570833333333333
2.07689336570759 0.575
2.07727121451031 0.579166666666667
2.09884349987305 0.583333333333333
2.11648838985299 0.5875
2.12369241932989 0.591666666666667
2.12409663818572 0.595833333333333
2.13687014680737 0.6
2.14506784928696 0.604166666666667
2.15800695939042 0.608333333333333
2.16957367534626 0.6125
2.18530882686283 0.616666666666667
2.18802150049477 0.620833333333333
2.19226365033388 0.625
2.20655362349035 0.629166666666667
2.24133924937937 0.633333333333333
2.24181692126439 0.6375
2.24892185608865 0.641666666666667
2.27883722695877 0.645833333333333
2.29524799165084 0.65
2.29728569954303 0.654166666666667
2.29937822070775 0.658333333333333
2.31677096049062 0.6625
2.37603891383661 0.666666666666667
2.38598562364576 0.670833333333333
2.38922494429159 0.675
2.42552553304922 0.679166666666667
2.43360976825998 0.683333333333333
2.46385782134351 0.6875
2.47878599259085 0.691666666666667
2.48695073640404 0.695833333333333
2.58889780199172 0.7
2.59541595675215 0.704166666666667
2.61752658609842 0.708333333333333
2.6320088792949 0.7125
2.63844108370157 0.716666666666667
2.66718430472529 0.720833333333333
2.69881363615299 0.725
2.70190885381112 0.729166666666667
2.72426536765875 0.733333333333333
2.73399762220051 0.7375
2.75535325192557 0.741666666666667
2.89292947230687 0.745833333333333
2.94153925558748 0.75
2.97817395558912 0.754166666666667
2.98486405868834 0.758333333333333
3.04584608889468 0.7625
3.06789871317799 0.766666666666667
3.07023086566189 0.770833333333333
3.07259446076202 0.775
3.07993363923707 0.779166666666667
3.08039620312242 0.783333333333333
3.12657674363959 0.7875
3.1339102484291 0.791666666666667
3.24704729851773 0.795833333333333
3.24989208563586 0.8
3.29715044864661 0.804166666666667
3.30029043955708 0.808333333333333
3.32125804185396 0.8125
3.3384657613275 0.816666666666667
3.35705727503956 0.820833333333333
3.37422779640192 0.825
3.44631767545669 0.829166666666667
3.47910273451737 0.833333333333333
3.49412091263207 0.8375
3.50366229457609 0.841666666666667
3.68600021819216 0.845833333333333
3.72434725956291 0.85
3.8128558986792 0.854166666666667
3.93137087503813 0.858333333333333
3.97214446944526 0.8625
3.98975131911903 0.866666666666667
3.99325292000613 0.870833333333333
4.06011849245747 0.875
4.16462060016959 0.879166666666667
4.20581029600615 0.883333333333333
4.30747210365642 0.8875
4.34414131794124 0.891666666666667
4.55038825288581 0.895833333333333
4.57300085791655 0.9
4.69593423019184 0.904166666666667
4.76809628137079 0.908333333333333
4.86873852331675 0.9125
4.93305555101399 0.916666666666667
5.05863727997299 0.920833333333333
5.11015225307056 0.925
5.13290317693837 0.929166666666667
5.1562895731075 0.933333333333333
5.26237321217531 0.9375
5.58788569293829 0.941666666666667
5.61902772830352 0.945833333333333
5.70909716045429 0.95
5.77065765333604 0.954166666666667
5.86731017867695 0.958333333333333
6.01308450881153 0.9625
6.11542628320703 0.966666666666667
6.40799519655997 0.970833333333333
7.24958365896767 0.975
7.39168951158165 0.979166666666667
7.53229091316541 0.983333333333333
7.60402414316299 0.9875
7.74116196204997 0.991666666666667
9.59834256223681 0.995833333333333
};
\addplot [thick,  dashed, forestgreen4416044]
table {%
1.18255999798386 0
1.18255999800108 0.00416666666666667
1.1825599981565 0.00833333333333333
1.18255999822475 0.0125
1.1825599982773 0.0166666666666667
1.18255999831313 0.0208333333333333
1.18255999843567 0.025
1.18255999847206 0.0291666666666667
1.18255999849731 0.0333333333333333
1.18255999851853 0.0375
1.18255999852776 0.0416666666666667
1.18255999866396 0.0458333333333333
1.18255999867271 0.05
1.1825599986778 0.0541666666666667
1.18255999884853 0.0583333333333333
1.18255999885569 0.0625
1.18255999886024 0.0666666666666667
1.18255999887227 0.0708333333333333
1.18255999891552 0.075
1.18255999892003 0.0791666666666667
1.18255999897127 0.0833333333333333
1.18255999899752 0.0875
1.18255999902866 0.0916666666666667
1.18255999903074 0.0958333333333333
1.18255999903109 0.1
1.18255999905471 0.104166666666667
1.18255999906286 0.108333333333333
1.18255999908642 0.1125
1.18255999913217 0.116666666666667
1.18255999917999 0.120833333333333
1.18255999920198 0.125
1.18255999924481 0.129166666666667
1.18255999927544 0.133333333333333
1.18255999931546 0.1375
1.18255999934016 0.141666666666667
1.18255999935726 0.145833333333333
1.18255999940622 0.15
1.1825599994142 0.154166666666667
1.1825599995115 0.158333333333333
1.18255999953191 0.1625
1.18255999955812 0.166666666666667
1.18255999956928 0.170833333333333
1.18255999958844 0.175
1.18255999963396 0.179166666666667
1.1825599996361 0.183333333333333
1.18255999967241 0.1875
1.18255999967834 0.191666666666667
1.18255999968906 0.195833333333333
1.18255999969666 0.2
1.18255999973202 0.204166666666667
1.18255999973959 0.208333333333333
1.18255999979911 0.2125
1.18255999981631 0.216666666666667
1.18255999984606 0.220833333333333
1.18255999986511 0.225
1.18255999989433 0.229166666666667
1.18255999989923 0.233333333333333
1.18255999990688 0.2375
1.18256000002345 0.241666666666667
1.18256000006269 0.245833333333333
1.18256000007927 0.25
1.18256000012844 0.254166666666667
1.18256000014936 0.258333333333333
1.18256000018954 0.2625
1.18256000020516 0.266666666666667
1.18256000025177 0.270833333333333
1.18256000035523 0.275
1.18256000035627 0.279166666666667
1.18256000035868 0.283333333333333
1.18256000041792 0.2875
1.18256000046804 0.291666666666667
1.18256000047438 0.295833333333333
1.18256000049262 0.3
1.18256000049698 0.304166666666667
1.18256000059905 0.308333333333333
1.18256000064042 0.3125
1.18256000067138 0.316666666666667
1.18256000074817 0.320833333333333
1.18256000075296 0.325
1.18256000093268 0.329166666666667
1.18256000094927 0.333333333333333
1.18256000100471 0.3375
1.18256000101118 0.341666666666667
1.18256000101179 0.345833333333333
1.18256000127203 0.35
1.18256000129964 0.354166666666667
1.1825600013207 0.358333333333333
1.1825600013257 0.3625
1.1825600013635 0.366666666666667
1.18256000139175 0.370833333333333
1.18256000151567 0.375
1.1825600015601 0.379166666666667
1.18256000156771 0.383333333333333
1.18256000176172 0.3875
1.1825600018757 0.391666666666667
1.1825600019487 0.395833333333333
1.18256000203069 0.4
1.18256000209423 0.404166666666667
1.18256000224322 0.408333333333333
1.18256000234992 0.4125
1.18256000249214 0.416666666666667
1.18256000252854 0.420833333333333
1.18256000259254 0.425
1.18256000287409 0.429166666666667
1.18256000294114 0.433333333333333
1.18256000295104 0.4375
1.18256000301726 0.441666666666667
1.1825600030564 0.445833333333333
1.18256000312455 0.45
1.18256000327545 0.454166666666667
1.18256000351292 0.458333333333333
1.18256000359554 0.4625
1.18256000364152 0.466666666666667
1.18256000365439 0.470833333333333
1.18256000375145 0.475
1.18256000378917 0.479166666666667
1.18256000384069 0.483333333333333
1.18256000396451 0.4875
1.18256000409895 0.491666666666667
1.18256000417093 0.495833333333333
1.18256000421535 0.5
1.1825600044528 0.504166666666667
1.18256000466767 0.508333333333333
1.18256000507642 0.5125
1.18256000536601 0.516666666666667
1.18256000541266 0.520833333333333
1.1825600055742 0.525
1.18256000563895 0.529166666666667
1.18256000566206 0.533333333333333
1.18256000576906 0.5375
1.18256000604407 0.541666666666667
1.18256000646468 0.545833333333333
1.18256000652221 0.55
1.1825600068327 0.554166666666667
1.18256000693639 0.558333333333333
1.18256000698658 0.5625
1.18256000702754 0.566666666666667
1.18256000748357 0.570833333333333
1.18256000765819 0.575
1.18256000777331 0.579166666666667
1.18256000812986 0.583333333333333
1.18256000824615 0.5875
1.18256000831079 0.591666666666667
1.18256000889802 0.595833333333333
1.1825600090571 0.6
1.182560009873 0.604166666666667
1.18256000989973 0.608333333333333
1.18256000998565 0.6125
1.18256001005617 0.616666666666667
1.18256001016714 0.620833333333333
1.18256001080756 0.625
1.18256001096041 0.629166666666667
1.18256001170392 0.633333333333333
1.18256001259788 0.6375
1.1825600126525 0.641666666666667
1.18256001265595 0.645833333333333
1.18256001321034 0.65
1.18256001392062 0.654166666666667
1.18256001626695 0.658333333333333
1.1825600179237 0.6625
1.18256001913673 0.666666666666667
1.18256001920421 0.670833333333333
1.18256002756084 0.675
1.1825600351002 0.679166666666667
1.18256004546185 0.683333333333333
1.18256006440112 0.6875
1.18256007361017 0.691666666666667
1.18256008269326 0.695833333333333
1.18256009765356 0.7
1.18256015174101 0.704166666666667
1.18256015624076 0.708333333333333
1.18256015687994 0.7125
1.18256018632888 0.716666666666667
1.18256018913275 0.720833333333333
1.18256043015355 0.725
1.18257505010108 0.729166666666667
1.24002559300867 0.733333333333333
1.24122960371702 0.7375
1.27846285355272 0.741666666666667
1.28966704751778 0.745833333333333
1.29120971775572 0.75
1.3122986260131 0.754166666666667
1.34238802560456 0.758333333333333
1.3471040309982 0.7625
1.35162308937511 0.766666666666667
1.39705282531086 0.770833333333333
1.40478468627935 0.775
1.4152223739647 0.779166666666667
1.42115783742503 0.783333333333333
1.42273205415777 0.7875
1.42370539802034 0.791666666666667
1.42601858552938 0.795833333333333
1.42704731082078 0.8
1.44950194505021 0.804166666666667
1.47009703041998 0.808333333333333
1.48393641113643 0.8125
1.48624256229592 0.816666666666667
1.50903060623042 0.820833333333333
1.53123695144965 0.825
1.54135243981281 0.829166666666667
1.62166275529386 0.833333333333333
1.67137533433976 0.8375
1.70514342793072 0.841666666666667
1.72746628730671 0.845833333333333
1.73029008633685 0.85
1.76747087863063 0.854166666666667
1.76762109466122 0.858333333333333
1.77451530790116 0.8625
1.79610928384706 0.866666666666667
1.80365194818946 0.870833333333333
1.86449245497282 0.875
1.8761828011627 0.879166666666667
1.88791222525689 0.883333333333333
1.90747427782903 0.8875
1.96372995802425 0.891666666666667
1.9713992602206 0.895833333333333
2.00698154012749 0.9
2.0255984826798 0.904166666666667
2.0316845627764 0.908333333333333
2.05113295792306 0.9125
2.06039671443448 0.916666666666667
2.08918281682673 0.920833333333333
2.16523445362227 0.925
2.17203013127068 0.929166666666667
2.18047502266725 0.933333333333333
2.41503421240542 0.9375
2.43663716444442 0.941666666666667
2.58783322759133 0.945833333333333
2.59395694820873 0.95
2.63449102745174 0.954166666666667
2.76996169495686 0.958333333333333
2.9956061614729 0.9625
3.00067665902499 0.966666666666667
3.1759964498249 0.970833333333333
3.18825631931496 0.975
3.46663392214009 0.979166666666667
3.53732121162535 0.983333333333333
3.67571418711761 0.9875
3.71277909431287 0.991666666666667
3.84410030776789 0.995833333333333
};


==> figures/techtile/rx-cdf-non-coherent.tex <==
\addplot [thick, steelblue31119180]
table {%
1.18255999999952 0
1.32827231911372 0.00416666666666667
1.33907083228939 0.00833333333333333
1.38792673056771 0.0125
1.38897685494514 0.0166666666666667
1.46617236114133 0.0208333333333333
1.51380296801145 0.025
1.52857885242845 0.0291666666666667
1.55117839647739 0.0333333333333333
1.57800666878267 0.0375
1.59663520275956 0.0416666666666667
1.60804738523503 0.0458333333333333
1.6186773992326 0.05
1.64402694101644 0.0541666666666667
1.70376727484975 0.0583333333333333
1.71400677386776 0.0625
1.71586264714172 0.0666666666666667
1.71971103705536 0.0708333333333333
1.75963941392738 0.075
1.80414630972709 0.0791666666666667
1.84102939547275 0.0833333333333333
1.85927551119518 0.0875
1.86555885714258 0.0916666666666667
1.86896427524778 0.0958333333333333
1.87350308967514 0.1
1.89518872317871 0.104166666666667
1.90232499148468 0.108333333333333
1.96244863552717 0.1125
1.97239173295661 0.116666666666667
1.98009631490445 0.120833333333333
2.00950356752257 0.125
2.01375428175213 0.129166666666667
2.01980239648071 0.133333333333333
2.07209618472921 0.1375
2.07439732358488 0.141666666666667
2.08737642950931 0.145833333333333
2.09840630184564 0.15
2.11220700929539 0.154166666666667
2.12859760748878 0.158333333333333
2.15801226967494 0.1625
2.16006436294319 0.166666666666667
2.19564342019777 0.170833333333333
2.21116858600785 0.175
2.21557441608787 0.179166666666667
2.22582349558207 0.183333333333333
2.23821923929148 0.1875
2.26313800277414 0.191666666666667
2.27697615359847 0.195833333333333
2.27909011761838 0.2
2.29531843693817 0.204166666666667
2.30146841996896 0.208333333333333
2.32863832156989 0.2125
2.35483129925497 0.216666666666667
2.35980091097435 0.220833333333333
2.37472802811684 0.225
2.42162347085191 0.229166666666667
2.4244652637889 0.233333333333333
2.45417239110719 0.2375
2.46301756064258 0.241666666666667
2.47830162268452 0.245833333333333
2.47839348334809 0.25
2.48417609545519 0.254166666666667
2.4904929782619 0.258333333333333
2.49673019400878 0.2625
2.50754914685938 0.266666666666667
2.51921038986816 0.270833333333333
2.52933663522634 0.275
2.56360473018204 0.279166666666667
2.56475045878865 0.283333333333333
2.57852331967505 0.2875
2.58838708453561 0.291666666666667
2.63209125462924 0.295833333333333
2.64058908835972 0.3
2.64921164106288 0.304166666666667
2.65692781696545 0.308333333333333
2.70602386072098 0.3125
2.71022328201349 0.316666666666667
2.72148545938534 0.320833333333333
2.74006032428186 0.325
2.74385457017726 0.329166666666667
2.79352484500716 0.333333333333333
2.79883144171385 0.3375
2.81946323617208 0.341666666666667
2.83829753272995 0.345833333333333
2.8499591685185 0.35
2.85476183344249 0.354166666666667
2.87520129551714 0.358333333333333
2.88189269481607 0.3625
2.88922458362036 0.366666666666667
2.94582444191343 0.370833333333333
2.94864495743567 0.375
2.99198066667794 0.379166666666667
3.03317711758014 0.383333333333333
3.04323503596635 0.3875
3.05389478187807 0.391666666666667
3.06620378529269 0.395833333333333
3.06905765400645 0.4
3.07223486013939 0.404166666666667
3.11067713545608 0.408333333333333
3.12554184686414 0.4125
3.13159218964277 0.416666666666667
3.13422120462032 0.420833333333333
3.14653127836562 0.425
3.15562571638874 0.429166666666667
3.16106172211089 0.433333333333333
3.18042029831063 0.4375
3.20137860098421 0.441666666666667
3.20393486852467 0.445833333333333
3.21466617155215 0.45
3.2365624605036 0.454166666666667
3.24853304254403 0.458333333333333
3.26121446354579 0.4625
3.2862876383411 0.466666666666667
3.30007282127337 0.470833333333333
3.36558176654841 0.475
3.37118475715919 0.479166666666667
3.38747528550362 0.483333333333333
3.39037834188817 0.4875
3.39610337528802 0.491666666666667
3.39927199966858 0.495833333333333
3.40420562911863 0.5
3.40598338442882 0.504166666666667
3.41318291102681 0.508333333333333
3.43206804837617 0.5125
3.43732206720812 0.516666666666667
3.50902994815304 0.520833333333333
3.52721267511904 0.525
3.54226838016337 0.529166666666667
3.54918746523941 0.533333333333333
3.5834779693636 0.5375
3.64480282734355 0.541666666666667
3.65859685592835 0.545833333333333
3.6674894749836 0.55
3.71575262656417 0.554166666666667
3.78343838974233 0.558333333333333
3.81987491781751 0.5625
3.82019725762357 0.566666666666667
3.86698824141005 0.570833333333333
3.91353864711813 0.575
3.93921725603935 0.579166666666667
3.9469327106072 0.583333333333333
3.96191228618061 0.5875
3.98457227445812 0.591666666666667
3.98893581453387 0.595833333333333
3.99708814333906 0.6
4.0117176838887 0.604166666666667
4.02459553315344 0.608333333333333
4.02981108255581 0.6125
4.0399257145901 0.616666666666667
4.04565002237248 0.620833333333333
4.04977487961217 0.625
4.05397482768245 0.629166666666667
4.08657597827821 0.633333333333333
4.10101776955813 0.6375
4.10372909426608 0.641666666666667
4.10921545410085 0.645833333333333
4.11623128117311 0.65
4.13565645152029 0.654166666666667
4.21745111090691 0.658333333333333
4.22393151510456 0.6625
4.26395406401603 0.666666666666667
4.26899805855741 0.670833333333333
4.30965129954318 0.675
4.3206250775485 0.679166666666667
4.35739812019839 0.683333333333333
4.39017526133225 0.6875
4.40017812328611 0.691666666666667
4.41403580106275 0.695833333333333
4.47712757622389 0.7
4.49221506991467 0.704166666666667
4.53188356416235 0.708333333333333
4.59251628535885 0.7125
4.59429121116388 0.716666666666667
4.61639256609506 0.720833333333333
4.71268090469455 0.725
4.7734633072255 0.729166666666667
4.77903009692797 0.733333333333333
4.80227979118274 0.7375
4.87680851556464 0.741666666666667
4.92903309174134 0.745833333333333
4.95067840795333 0.75
4.96354781156142 0.754166666666667
4.9711544287029 0.758333333333333
5.1411959615098 0.7625
5.14255471746672 0.766666666666667
5.18383014849955 0.770833333333333
5.25568709475705 0.775
5.26620668251811 0.779166666666667
5.26767458023318 0.783333333333333
5.3315697235798 0.7875
5.33936535568128 0.791666666666667
5.34663833556355 0.795833333333333
5.37127154094438 0.8
5.56091074924683 0.804166666666667
5.61717511638809 0.808333333333333
5.63542558127481 0.8125
5.65756399127257 0.816666666666667
5.7206482087347 0.820833333333333
6.00759015987708 0.825
6.01966128021945 0.829166666666667
6.22112708617542 0.833333333333333
6.32408314628538 0.8375
6.39138468617283 0.841666666666667
6.41098709549779 0.845833333333333
6.43679074662068 0.85
6.47536872970535 0.854166666666667
6.85416868513487 0.858333333333333
6.99560802943451 0.8625
7.12724052724564 0.866666666666667
7.13263560210623 0.870833333333333
7.15445270822515 0.875
7.3474165071465 0.879166666666667
7.37869179525189 0.883333333333333
7.41823673911437 0.8875
7.79367573536708 0.891666666666667
7.94349000646494 0.895833333333333
8.02224926292908 0.9
8.30849317145762 0.904166666666667
8.38805429026852 0.908333333333333
8.46455840118459 0.9125
8.49815445154439 0.916666666666667
8.76603875939539 0.920833333333333
8.94716172020719 0.925
9.07803074935923 0.929166666666667
9.37057541024994 0.933333333333333
9.37092726236143 0.9375
10.362598983122 0.941666666666667
10.3797438695581 0.945833333333333
10.413149109488 0.95
11.6160447886019 0.954166666666667
11.8879489299952 0.958333333333333
12.1940782183618 0.9625
12.3996997699275 0.966666666666667
12.7041769141876 0.970833333333333
12.8073359806264 0.975
13.6129689767341 0.979166666666667
13.7453931879059 0.983333333333333
16.5860818932916 0.9875
17.4747773323691 0.991666666666667
18.9869698338156 0.995833333333333
};
\addplot [thick, darkorange25512714]
table {%
1.18256 0
1.18256 0.00416666666666667
1.18256 0.00833333333333333
1.18256 0.0125
1.18256000000003 0.0166666666666667
1.18256000000005 0.0208333333333333
1.18382771122078 0.025
1.1857664313 0.0291666666666667
1.18611292512463 0.0333333333333333
1.19226424113367 0.0375
1.19276956253358 0.0416666666666667
1.19333043229009 0.0458333333333333
1.20545032181945 0.05
1.20672059001811 0.0541666666666667
1.21050741209311 0.0583333333333333
1.21574813918508 0.0625
1.22681437333545 0.0666666666666667
1.23884771570445 0.0708333333333333
1.2467896450984 0.075
1.24681627624072 0.0791666666666667
1.25873530955617 0.0833333333333333
1.2633042295148 0.0875
1.26410214020033 0.0916666666666667
1.27346818745211 0.0958333333333333
1.28169530406829 0.1
1.29036235477999 0.104166666666667
1.30021467823552 0.108333333333333
1.30556889450464 0.1125
1.30765979373597 0.116666666666667
1.31065444846706 0.120833333333333
1.31227541533101 0.125
1.31299267743149 0.129166666666667
1.32230502694299 0.133333333333333
1.32605433983901 0.1375
1.32676449844833 0.141666666666667
1.34647449835862 0.145833333333333
1.36971055264793 0.15
1.38782543327998 0.154166666666667
1.38867189437774 0.158333333333333
1.41116214617415 0.1625
1.41456178675973 0.166666666666667
1.41652000563212 0.170833333333333
1.4218107328687 0.175
1.44136640312028 0.179166666666667
1.45132267010098 0.183333333333333
1.46088919396769 0.1875
1.46381397485122 0.191666666666667
1.46525564124846 0.195833333333333
1.46794583702801 0.2
1.46925975917667 0.204166666666667
1.46951848247005 0.208333333333333
1.47378587260478 0.2125
1.48102096466772 0.216666666666667
1.4946869741956 0.220833333333333
1.49845050758693 0.225
1.50159397104923 0.229166666666667
1.50329922939554 0.233333333333333
1.50606221911352 0.2375
1.5417170981777 0.241666666666667
1.55863328585445 0.245833333333333
1.57189326476363 0.25
1.57404835847562 0.254166666666667
1.57998058963435 0.258333333333333
1.5809696226928 0.2625
1.6091343386435 0.266666666666667
1.61491727640781 0.270833333333333
1.616183178467 0.275
1.61761794559292 0.279166666666667
1.64539320824416 0.283333333333333
1.64710740742658 0.2875
1.65626264077327 0.291666666666667
1.66011392447244 0.295833333333333
1.67898676412208 0.3
1.68003640332439 0.304166666666667
1.70181867730636 0.308333333333333
1.70903036619969 0.3125
1.71746669810489 0.316666666666667
1.74239584633325 0.320833333333333
1.75435897576818 0.325
1.75466722710566 0.329166666666667
1.76265459217482 0.333333333333333
1.76316977626984 0.3375
1.76451852195838 0.341666666666667
1.77439352824891 0.345833333333333
1.77503898688081 0.35
1.79069437119767 0.354166666666667
1.81787207941193 0.358333333333333
1.81869262889579 0.3625
1.82055706226457 0.366666666666667
1.82644114235446 0.370833333333333
1.82683180429909 0.375
1.82800373643546 0.379166666666667
1.83273424932275 0.383333333333333
1.83810052653706 0.3875
1.84582720123315 0.391666666666667
1.85367111205955 0.395833333333333
1.86966038041539 0.4
1.87225919296153 0.404166666666667
1.87272830919256 0.408333333333333
1.88984160035488 0.4125
1.90419452827123 0.416666666666667
1.9099715921123 0.420833333333333
1.91517855794854 0.425
1.91892470358003 0.429166666666667
1.95382412769879 0.433333333333333
1.95460449978825 0.4375
1.95695921425843 0.441666666666667
1.96133123160042 0.445833333333333
1.96626642747847 0.45
1.96692073527757 0.454166666666667
2.00070319186663 0.458333333333333
2.00617951600881 0.4625
2.01726929532438 0.466666666666667
2.03748315133232 0.470833333333333
2.06779554377745 0.475
2.13021365281797 0.479166666666667
2.16391014350079 0.483333333333333
2.16446925258286 0.4875
2.16968535539346 0.491666666666667
2.17686071395129 0.495833333333333
2.18112408318241 0.5
2.20379812558228 0.504166666666667
2.20645108816856 0.508333333333333
2.20918896749046 0.5125
2.21386094136323 0.516666666666667
2.23877993319773 0.520833333333333
2.24063680175579 0.525
2.25595894417471 0.529166666666667
2.25658434777303 0.533333333333333
2.26044744813777 0.5375
2.29724748677919 0.541666666666667
2.32308265809119 0.545833333333333
2.32780814080869 0.55
2.33483823991746 0.554166666666667
2.35002525555964 0.558333333333333
2.35919773633149 0.5625
2.36342560149138 0.566666666666667
2.37312271194246 0.570833333333333
2.37539083650005 0.575
2.39697933418595 0.579166666666667
2.40115617888934 0.583333333333333
2.42195994714609 0.5875
2.42863208431871 0.591666666666667
2.42954414287028 0.595833333333333
2.44998626839604 0.6
2.46633913889873 0.604166666666667
2.46999885907532 0.608333333333333
2.47087430950225 0.6125
2.47330599332457 0.616666666666667
2.52373920941761 0.620833333333333
2.53129514627783 0.625
2.54183936541044 0.629166666666667
2.55535741812654 0.633333333333333
2.59905542774841 0.6375
2.60857225666694 0.641666666666667
2.61477772019468 0.645833333333333
2.62379028441505 0.65
2.67585322155543 0.654166666666667
2.68418172571469 0.658333333333333
2.68496882458691 0.6625
2.68838497931014 0.666666666666667
2.69286615503811 0.670833333333333
2.70276261101011 0.675
2.73201556884441 0.679166666666667
2.7442922014646 0.683333333333333
2.75128699971897 0.6875
2.75598488183879 0.691666666666667
2.77341376062467 0.695833333333333
2.77529930139962 0.7
2.78449482391906 0.704166666666667
2.80102787084672 0.708333333333333
2.82682775239585 0.7125
2.83579783340458 0.716666666666667
2.87211373593858 0.720833333333333
2.90351045591057 0.725
2.90751975737202 0.729166666666667
2.93860673446753 0.733333333333333
2.94998936631722 0.7375
3.0195630626493 0.741666666666667
3.03051781799998 0.745833333333333
3.12652595242919 0.75
3.19488572523691 0.754166666666667
3.24074643833619 0.758333333333333
3.24124008872988 0.7625
3.31017165229169 0.766666666666667
3.36523948987263 0.770833333333333
3.42216516106037 0.775
3.43505417063808 0.779166666666667
3.48700419674735 0.783333333333333
3.51658054002747 0.7875
3.61177533769684 0.791666666666667
3.67682407970347 0.795833333333333
3.69129476234498 0.8
3.7157716311056 0.804166666666667
3.72129954357951 0.808333333333333
3.80390850068502 0.8125
3.81339689556035 0.816666666666667
3.86277455794026 0.820833333333333
4.00604069011664 0.825
4.01694762771706 0.829166666666667
4.14489354458689 0.833333333333333
4.16472119739422 0.8375
4.19723546107579 0.841666666666667
4.26436840655655 0.845833333333333
4.29885726916894 0.85
4.29971362247755 0.854166666666667
4.3026221057639 0.858333333333333
4.50640978684023 0.8625
4.68955869299817 0.866666666666667
4.76673349038864 0.870833333333333
4.77297366530237 0.875
4.8154045778794 0.879166666666667
4.8937718166853 0.883333333333333
4.95371241521054 0.8875
5.11414198593355 0.891666666666667
5.18229884045762 0.895833333333333
5.25083210301571 0.9
5.33673387790864 0.904166666666667
5.57652159412811 0.908333333333333
5.8869107566799 0.9125
6.01899345241773 0.916666666666667
6.06600709373974 0.920833333333333
6.3790692417528 0.925
6.50460953785731 0.929166666666667
6.72438883166853 0.933333333333333
7.24540954713657 0.9375
7.56186381020415 0.941666666666667
7.96822269600592 0.945833333333333
8.1199390295231 0.95
8.19359434296691 0.954166666666667
8.43615300534094 0.958333333333333
8.60339062013154 0.9625
8.80464483403162 0.966666666666667
9.32645793432419 0.970833333333333
10.4464631773139 0.975
11.9402520920406 0.979166666666667
15.0207365004969 0.983333333333333
15.325619677642 0.9875
20.1017363072538 0.991666666666667
25.6062445662876 0.995833333333333
};
\addplot [thick, forestgreen4416044]
table {%
1.18255999999983 0
1.18255999999983 0.00416666666666667
1.18255999999983 0.00833333333333333
1.18255999999983 0.0125
1.18255999999985 0.0166666666666667
1.18255999999986 0.0208333333333333
1.18255999999986 0.025
1.18255999999987 0.0291666666666667
1.18256000000008 0.0333333333333333
1.18269893464733 0.0375
1.18522647239195 0.0416666666666667
1.18546295792059 0.0458333333333333
1.18624945783578 0.05
1.18664591449884 0.0541666666666667
1.18666756207995 0.0583333333333333
1.18681620213839 0.0625
1.18908452146277 0.0666666666666667
1.18940037126115 0.0708333333333333
1.18984329159924 0.075
1.19011365194424 0.0791666666666667
1.19157781642809 0.0833333333333333
1.19182876133386 0.0875
1.2007275706701 0.0916666666666667
1.20164593672116 0.0958333333333333
1.21159078565922 0.1
1.21191918564131 0.104166666666667
1.22673169814031 0.108333333333333
1.22821414782836 0.1125
1.2402293928058 0.116666666666667
1.2405821975982 0.120833333333333
1.25064166098589 0.125
1.2506706620188 0.129166666666667
1.25821291583162 0.133333333333333
1.25887064068068 0.1375
1.26027104976718 0.141666666666667
1.26221680840508 0.145833333333333
1.27011788801878 0.15
1.27041375814531 0.154166666666667
1.286125935504 0.158333333333333
1.28615042505668 0.1625
1.28966187147098 0.166666666666667
1.28982390949596 0.170833333333333
1.29232509951717 0.175
1.29445675432215 0.179166666666667
1.30125621170519 0.183333333333333
1.30262319870561 0.1875
1.31019475872053 0.191666666666667
1.31211804357958 0.195833333333333
1.44721224719971 0.2
1.44811952301138 0.204166666666667
1.4483206964467 0.208333333333333
1.44915833874071 0.2125
1.45009572544475 0.216666666666667
1.450473838271 0.220833333333333
1.45606836644403 0.225
1.45703760372353 0.229166666666667
1.46010030571398 0.233333333333333
1.46124213145868 0.2375
1.46643846715763 0.241666666666667
1.46657493291872 0.245833333333333
1.47229430810003 0.25
1.47351798180944 0.254166666666667
1.47427669622379 0.258333333333333
1.4743157858345 0.2625
1.48206787684497 0.266666666666667
1.48230840719705 0.270833333333333
1.48512452614023 0.275
1.48562357714116 0.279166666666667
1.50196825283049 0.283333333333333
1.50295164337569 0.2875
1.52733473145155 0.291666666666667
1.53037624266723 0.295833333333333
1.57135556994444 0.3
1.57176083731805 0.304166666666667
1.59006004955775 0.308333333333333
1.59343343335828 0.3125
1.59579947528408 0.316666666666667
1.59893519354645 0.320833333333333
1.60847675050477 0.325
1.61204127778801 0.329166666666667
1.65454769214763 0.333333333333333
1.65545055631254 0.3375
1.69892253105478 0.341666666666667
1.70183769781167 0.345833333333333
1.70937451581808 0.35
1.71398022944161 0.354166666666667
1.72127438186175 0.358333333333333
1.72448015182069 0.3625
1.7256407236831 0.366666666666667
1.72851096729887 0.370833333333333
1.75170384801036 0.375
1.75221147796266 0.379166666666667
1.75390220391821 0.383333333333333
1.75673470903212 0.3875
1.75957251823409 0.391666666666667
1.76348943697216 0.395833333333333
1.76924996073165 0.4
1.77012700494451 0.404166666666667
1.7707599294346 0.408333333333333
1.77373390413425 0.4125
1.77509564607621 0.416666666666667
1.77694734771888 0.420833333333333
1.78334736728728 0.425
1.78498908246944 0.429166666666667
1.78561267748577 0.433333333333333
1.78909099882862 0.4375
1.79623424634749 0.441666666666667
1.80099546012953 0.445833333333333
1.82882435350939 0.45
1.83177113584544 0.454166666666667
1.84855886884847 0.458333333333333
1.84982427684052 0.4625
1.85025249749776 0.466666666666667
1.85589010834751 0.470833333333333
1.87609144201361 0.475
1.88094248796437 0.479166666666667
1.88508457524186 0.483333333333333
1.89103965975649 0.4875
1.89132506100601 0.491666666666667
1.89571165979163 0.495833333333333
1.99603410707113 0.5
1.99905840808612 0.504166666666667
2.05604926562141 0.508333333333333
2.06040364972962 0.5125
2.06992860499825 0.516666666666667
2.07219286283508 0.520833333333333
2.07958387916018 0.525
2.08129612770964 0.529166666666667
2.08604933697367 0.533333333333333
2.09255433573657 0.5375
2.09548114845756 0.541666666666667
2.10026827963989 0.545833333333333
2.12534139093436 0.55
2.13251229911997 0.554166666666667
2.17534475676082 0.558333333333333
2.19278023141551 0.5625
2.19568790084495 0.566666666666667
2.20648097529403 0.570833333333333
2.20667365224397 0.575
2.20878083499253 0.579166666666667
2.21739636621076 0.583333333333333
2.24344420071994 0.5875
2.2473868514003 0.591666666666667
2.25554671937275 0.595833333333333
2.2702650610444 0.6
2.27211999340666 0.604166666666667
2.27391906751398 0.608333333333333
2.27522241943322 0.6125
2.27734486183584 0.616666666666667
2.27830776923093 0.620833333333333
2.29255705035522 0.625
2.29452303441925 0.629166666666667
2.29955710016692 0.633333333333333
2.30547444898337 0.6375
2.3055110433555 0.641666666666667
2.30973150432084 0.645833333333333
2.31469812833407 0.65
2.31515706408954 0.654166666666667
2.33199740951864 0.658333333333333
2.33757702949528 0.6625
2.37021379993626 0.666666666666667
2.39148723844922 0.670833333333333
2.39203853502111 0.675
2.39726863273364 0.679166666666667
2.39979104896388 0.683333333333333
2.40894040519906 0.6875
2.42548168652086 0.691666666666667
2.42749267371343 0.695833333333333
2.46200111328582 0.7
2.46227238817428 0.704166666666667
2.46543686365745 0.708333333333333
2.47449424484916 0.7125
2.4752535804464 0.716666666666667
2.47606198695554 0.720833333333333
2.49201052449074 0.725
2.49385922521327 0.729166666666667
2.5081874201353 0.733333333333333
2.51264081855532 0.7375
2.51532380589395 0.741666666666667
2.51665826580944 0.745833333333333
2.51755816963025 0.75
2.55757559743361 0.754166666666667
2.55879493367609 0.758333333333333
2.558883316647 0.7625
2.57495986802397 0.766666666666667
2.61202756754575 0.770833333333333
2.61294087634247 0.775
2.61604329718971 0.779166666666667
2.62480157317242 0.783333333333333
2.66024670825447 0.7875
2.6971141590278 0.791666666666667
2.76987840014369 0.795833333333333
2.81353904720004 0.8
2.85043345379758 0.804166666666667
2.85508794918244 0.808333333333333
2.89575134934263 0.8125
2.89851691723678 0.816666666666667
2.90682142525704 0.820833333333333
2.95649894329604 0.825
2.96449139622268 0.829166666666667
3.05469915137931 0.833333333333333
3.08906280879134 0.8375
3.09945446956416 0.841666666666667
3.13016941664378 0.845833333333333
3.15909405357756 0.85
3.21539448765272 0.854166666666667
3.29524485034548 0.858333333333333
3.39231633613165 0.8625
3.39568198352112 0.866666666666667
3.53481478028602 0.870833333333333
3.57358784802165 0.875
3.59811230584217 0.879166666666667
3.68590360920356 0.883333333333333
3.68735633147348 0.8875
3.72160776627299 0.891666666666667
3.74586417387486 0.895833333333333
3.79241953722814 0.9
3.85070856155705 0.904166666666667
3.87471268123412 0.908333333333333
3.97663362567062 0.9125
3.99963446456273 0.916666666666667
4.05900738084917 0.920833333333333
4.07612265617514 0.925
4.07669689631073 0.929166666666667
4.19098393938193 0.933333333333333
4.2651113942154 0.9375
4.45987371170653 0.941666666666667
4.59517388691059 0.945833333333333
4.8350212139634 0.95
4.86778271658554 0.954166666666667
5.06898779721601 0.958333333333333
5.11840023645595 0.9625
5.16858548463419 0.966666666666667
5.2341281572047 0.970833333333333
5.46682586316353 0.975
5.57041382666462 0.979166666666667
6.26927609444177 0.983333333333333
6.44114123312638 0.9875
6.51271019394231 0.991666666666667
6.82710297144187 0.995833333333333
};

